Coupling Temperature Distribution with the Single Particle Model

The DFN (Doyle-Fuller-Newman) model is well know for being accurate and computationally expensive. In situations where temperature gradients are important (eg fast charging) it is desirable to couple the temperature dynamics within a battery into the DFN model. This leads to even greater computational complexity. Inspired by the work of Marquis et al [1] we present the derivation of a reduced-order model based on the DFN model with temperature in the macroscale. The complexity of the reduced-order model is characterised by the local temperature plus one internal electro-chemical dimension and the electrolyte dynamics is accounted for by a simple correction term.

==> Asymptotic_Expansion.tex <==
\subsection{Mat's calculations}
A 1D model is sought for the TSPMe, so the 1D version of the full model is presented here. The electric potential for the active electrode particles is homogenised as a source term for the temperature, lithium concentration and electric potential in the electrolyte.
\begin{equation}
\partial_{y} J_{\textrm{s}}=-\frac{3}{R}\,J
\end{equation}
Where $J_{\textrm{s}}$ is the homogenised current in the electrode particles and $R_{k}$ is the radius of the electrode particles in $k\in\{n,p\}$
The equations in the electrolyte for the electric potential and lithium concentration are:
\begin{equation}
\p_{t} c_{\textrm{e}}=\p_{y}\left(D_{\textrm{L}}\p_y c_{\textrm{e}}+F\mu_{\textrm{L}} \,J_{\textrm{e}}\right)+\frac{3J}{RF}
\end{equation}
\begin{equation}
\p_{y}\left( (D_{\textrm{L}}-D_{\textrm{A}})\p_y c_{\textrm{e}}+F(\mu_{\textrm{L}}+\mu_{\textrm{A}})J_{\textrm{e}}\right)+\frac{3J}{RF}=0
\end{equation}
The parameters $D_{\textrm{L}}$ and $D_{\textrm{A}}$ are mesoscale diffusivity parameters for the lithium ions and anions respectively and $\mu_{\textrm{L}},\mu_{\textrm{A}}$ are the mobilities of the lithium and anions. The variables are the lithium concentration in the electrolyte($c_{\textrm{e}}$) and the current in the electrolyte($J_{\textrm{e}}$).  
\newline
\noindent
\textbf{Boundary Conditions}
The electric potentials
\begin{equation}
J_\mathrm{s}\big|_{x=1-L_{\textrm{c}}}=0,\quad J_\mathrm{s}\big|_{x=1}=-{I},\quad J_\mathrm{s}\big|_{x=L_{\textrm{a}}}=-{I}.%,\quad\Phi_{s,a}(t,0)=0.
\end{equation}
Define ionic current as:
\begin{equation}
i_{\textrm{e}}=(D_{\textrm{L}}-D_{\textrm{A}})\p_{x}{c_{\textrm{e}}}+F(\mu_{\textrm{L}}+\mu_{\textrm{A}})c_{\textrm{e}}J_{\textrm{e}}
\end{equation}
The boundary conditions for the ionic current is:
\begin{equation}
i_{\textrm{e}}(0)=0,\quad i_{\textrm{e}}(1)=0,\quad i_{\textrm{e}}(L_{\textrm{a}})=-I=i_{\textrm{e}}(1-\Lp)
\end{equation}
\begin{equation}
i_{\textrm{e}}(t,L_{\textrm{a}})=-I,\quad i_{\textrm{e}}(t,L_{\textrm{a}}+L_{\textrm{s}})
\end{equation}
The voltage is now defined as:
\begin{equation}
V=\Phi_{\textrm{s}}(y=1)-\Phi_{\textrm{s}}(y=0)
\end{equation}
The potentials are defined by:
\begin{equation}
J_{\textrm{s}}=\poo{\Phi_{\textrm{s}}}{y},\quad J_{\textrm{e}}=\poo{\Phi_{\textrm{e}}}{y}
\end{equation}
The governing equation for $J_{\textrm{s}}$ can be rewritten as:
\begin{equation}
\p_{y}J_{\textrm{s}}=\p_{y}{i_{\textrm{e}}}
\end{equation}
This equation can be simply integrated to $J_{\textrm{s}}=i_{\textrm{e}}+C$, using the boundary condition at $y=L_{\textrm{a}}$ demonstrates $C=-I$ making the equation:
\begin{equation}
J_{\textrm{s}}=i_{\textrm{e}}-I
\end{equation}
The functions, $\ce,\Phie,\Phis,J$ are all expanded as a regular asymptotic expansion in $\varepsilon$, $f=f^{0}+\varepsilon f^{1}$. The lowest order equations are:
\begin{equation}
D_\mathrm{e}\p_{y}^{2}\ce^{0}=0,\quad \alphae\p_{y}^{2}\Phie^{0}=0,\quad \alphas\p_{y}^{2}\Phis^{0}=0
\end{equation}
The boundary terms become:
\begin{equation}
\p_{y}\ce^{0}=0\quad y=0,1,\quad \p_{y}\Phie^{0}=0\quad y=\Ln,1-\Lp,\p_{y}\Phis^{0}=0\quad\textrm{cell boundaries}
\end{equation}
The solutions to these equations are:
\begin{equation}
\ce^{0}=1,\quad\Phie^{0}=0,\quad\Phis\quad\textrm{function of t}
\end{equation}
The expansion for the overpotential, $\eta^{0}$, is
\begin{equation}
\eta^{0}=\Phis^{0}-\Phie^{0}-U_\mathrm{ocp}=\Phis^{0}-U_\mathrm{ocp}\Rightarrow \Phis^{0}=U_\mathrm{ocp}+\eta_{0}
\end{equation}
The Butler-Volmer equation indicates that $J$ is independent of $y$, so this yields a linear relationship between $J$ and $i(t,x)$ which is:
\begin{displaymath}
J_{0}=\left\{
\begin{array}{cc}
\frac{i(t,x)}{\Ln}    & 0<y<\Ln \\
0 &  \Ln<y<1-\Lp \\
-\frac{i(t,x)}{\Lp} & 1-\Lp<y<1
\end{array}\right.
\end{displaymath}
The expansion of the overpotential as an asymptotic series demonstrates $V_{0}=\eta_{0}(1)+U_\mathrm{ocp}(1)-\eta_{0}(0)-U_\mathrm{ocp}(0)$. 
Moving on to the next order, we obtain:
\begin{equation}
D_\mathrm{e}\p_{y}^{2}\ce^{1}=-J^{0},\quad \alphae\p_{y}^{2}\Phie^{1}=J^{0},\quad \alphas\p_{y}^{2}\Phis^{1}=J^{0}
\end{equation}
The boundary conditions are then:
\begin{equation}
\p_{y}\ce^{1}=0,\quad y=0,1,\quad\p_{y}\Phie^{1}=0\quad\textrm{cell boundaries},\quad \p_{y}\Phis^{1}=\mp J^{0},\quad y=\Ln,1-\Lp 
\end{equation}
The next stage is to compute the heat source terms. The relevant quantities for the computation of the heat source terms.
\begin{displaymath}
D_\mathrm{e}\p_{y}c_{e}^{1}=\left\{
\begin{array}{cc}
\frac{y\,i}{\Ln} & 0<y<\Ln \\
0 & \Ln<y<1-\Lp \\
\frac{(1-y)\,i}{\Lp} & 1-\Lp<y<1
\end{array}\right.
\quad\alphae\p_{y}\Phie^{1}=\left\{ 
\begin{array}{cc}
-\frac{i\,\xi\, y}{\Ln} & 0<y<\Ln \\
0 & \Ln < y<1-\Ln \\
\frac{i\,\xi (1-y)}{\Lp} & 1-\Lp<y<1
\end{array}\right.
\end{displaymath}
\begin{displaymath}
\alphas\p_{y}\Phis^{1}=\left\{
\begin{array}{cc}
\frac{i}{\Ln}(y-2\Ln) & 0<y<\Ln \\
0 & \Ln<y<1-\Lp \\
\frac{i}{\Lp}(1-y) & 1-\Lp<y<1
\end{array}\right.
\end{displaymath}
where $\xi=\nu\beta_\mathrm{e}/D_\mathrm{e}-1$

